Immersed Boundary-Conformal Isogeometric Method for Linear Elliptic Problems

We present a novel isogeometric method, namely the Immersed Boundary-Conformal Method (IBCM), that features a layer of discretization conformal to the boundary while employing a simple background mesh for the remaining domain. In this manner, we leverage the geometric flexibility of the immersed boundary method with the advantages of a conformal discretization, such as intuitive control of mesh resolution around the boundary, higher accuracy per degree of freedom, automatic satisfaction of interface kinematic conditions, and the ability to strongly impose Dirichlet boundary conditions. In the proposed method, starting with a boundary representation of a geometric model, we extrude it to obtain a corresponding conformal layer. Next, a given background B-spline mesh is cut with the conformal layer, leading to two disconnected regions: an exterior region and an interior region. Depending on the problem of interest, one of the two regions is selected to be coupled with the conformal layer through Nitsche's method. Such a construction involves Boolean operations such as difference and union, which therefore require proper stabilization to deal with arbitrarily cut elements. In this regard, we follow our precedent work called the minimal stabilization method [1]. In the end, we solve several 2D benchmark problems to demonstrate improved accuracy and expected convergence with IBCM. Two applications that involve complex geometries are also studied to show the potential of IBCM, including a spanner model and a fiber-reinforced composite model. Moreover, we demonstrate the effectiveness of IBCM in an application that exhibits boundary-layer phenomena.

==> extrusion.tex <==

%% How do we construct the conformal layer?
We aim for a conformal layer $\conformalLayer$ that (1) represents the boundary or interface $\interface$ exactly and (2) is consistent with the parameterization of $\interface$.
First, we define a target curve $\targetCurve$, which specifies the interface of $\conformalLayer$ to the interior region of the background domain $\backDomainIn$; see Fig. \ref{fig:boundary_type}(a).


%% State-of-the-art of offsets
From a geometric point of view, the most natural choice for $\targetCurve$ is an offset to $\interface$.
Offset curves are defined as the locus of points that are at a constant distance $d$ along the normal vector from the so-called progenitor curve \cite{Hoschek1992b,patrikalakis2009b},
and there are several techniques in the literature to generate them, see e.g.~\cite{Maekawa1999a,Pham1992a}.
%% Challenge of offset curves
In general, offset curves are more complex than the progenitor curve, and they may have cusps and may self-intersect locally or globally. 
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.8\columnwidth]{offsetExample}
    \caption{A progenitor curve (thick) and various offset curves (dashed) with different distance $d$.}
    \label{fig:offsetExample}
\end{figure}
These self-intersections are linked to the distance $d$ of the offset curve (see Fig.~\ref{fig:offsetExample}). 
In particular, local self-intersections occur in concave regions when the absolute value of $d$ exceeds the minimum radius of curvature, and global self-intersections occur when the distance between two distinct points on the progenitor curve is smaller than $2d$ \cite{patrikalakis2009b}.
Wallner et al.~\cite{WALLNER2001a} presented an approach to determine the maximal offset distance to avoid self-intersections.

%% offset curves for the conformal layer
To sum up, using offset curves for the construction of the conformal layer $\conformalLayer$ may imply that the parameterization from the target curve $\targetCurve$ does not match with the one from the interface $\interface$, especially when $d$ is large. 
In this case, $\conformalLayer$ may be constructed as a loft surface between $\interface$ and $\targetCurve$, where a superset of the knot vectors of $\interface$ and $\targetCurve$ define the resulting parameterization. 
%% drawbacks
This approach has some disadvantages: First, the final parameterization of $\conformalLayer$ is partly determined by the offset curve scheme, and second, $C^0$-continuities may be introduced when the offset curve has cusps or self-intersections that have been trimmed away.

%% what we do to match the parameterization
Fortunately, we are very flexible in the definition of the target curve $\targetCurve$ in terms of the distance $d$ and its shape. We will see related examples in Section \ref{sec:result}. Hence, we suggest the following procedure for the construction of $\conformalLayer$:
\begin{enumerate}
    \item Define $\targetCurve$ either by an offset curve or any other curve that does not intersect $\interface$ and is at least as smooth as $\interface$.
    \item Project the Greville points of $\interface$ onto $\targetCurve$.
    \item Use the projected Greville points to construct an approximation of $\targetCurve$ that has the same knot vector and degree as $\interface$.
\end{enumerate}
%
% Of course, the resulting approximation of $\targetCurve$ will deviate locally from $\targetCurve$. 
This Greville point projection allows a straightforward realization of the conformal layer $\conformalLayer$ as a parameterization-consistent extrusion of $\interface$. 

\vspace{+2mm}
\noindent \textbf{Remark 4}. If the target curve $\targetCurve$ is given by an offset curve. We first check if it has cusps or regions with high curvature, and replace them by rounded fillets to avoid that projected Greville points coincide.
\vspace{+2mm}

